DART: Disease-aware Image-Text Alignment and Self-correcting Re-alignment for Trustworthy Radiology Report Generation

The automatic generation of radiology reports has emerged as a promising solution to reduce a time-consuming task and accurately capture critical disease-relevant findings in X-ray images. Previous approaches for radiology report generation have shown impressive performance. However, there remains significant potential to improve accuracy by ensuring that retrieved reports contain disease-relevant findings similar to those in the X-ray images and by refining generated reports. In this study, we propose a Disease-aware image-text Alignment and self-correcting Re-alignment for Trustworthy radiology report generation (DART) framework. In the first stage, we generate initial reports based on image-to-text retrieval with disease-matching, embedding both images and texts in a shared embedding space through contrastive learning. This approach ensures the retrieval of reports with similar disease-relevant findings that closely align with the input X-ray images. In the second stage, we further enhance the initial reports by introducing a self-correction module that re-aligns them with the X-ray images. Our proposed framework achieves state-of-the-art results on two widely used benchmarks, surpassing previous approaches in both report generation and clinical efficacy metrics, thereby enhancing the trustworthiness of radiology reports.

==> rebuttal/table_CEmetric.tex <==
\begin{table}[]
\centering
\caption{An additional comparison in clinical efficacy (CE) metrics and disease classification performance on MIMIC-CXR.}
\label{rebuttal:cemetrics}
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{c|cccc}
\hline
% \multicolumn{5}{c}{Clinical Efficacy (CE) Metrics}                      \\\hline
Method          & F1    & Precision & Recall & AUC  \\ \hline
PPKED [21]     & -     & -         & -      & 0.80 \\
RGRG [33]      & 0.447 & 0.461     & 0.475  & -    \\
I3 + C2FD [49] & 0.473 & 0.465     & 0.482  & -    \\ \hline
DART (CE Metrics) & \textbf{0.533} & \textbf{0.520} & \textbf{0.546} & \textbf{0.86} \\
% \hline
% \hline
% \multicolumn{5}{c}{Performance of Disease Classifier}                      \\ \hline
% Model         & F1    & Precision & Recall & AUC  \\ \hline
(Disease Classification)    & (0.427) & (0.404)     & (0.506)  & (0.83) \\ \hline
\end{tabular}%
}
\end{table}

==> rebuttal/table_ablation.tex <==
\begin{table}[]
\centering
\caption{An additional ablation study for key components.}
% \caption{An additional ablation study to assess the impact of four key components: contrastive loss (CL), image-to-text retrieval (I2T), disease-matching constraint (DM), and self-correction (SC).}
\label{rebuttal:ablation}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccc|cccccc}
\hline
Setting & CL         & I2T        & DM         & SC         & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & RG-L  & METEOR \\ \hline
BASE    & -          & -          & -          & -          & 0.371  & 0.233  & 0.157  & 0.111  & 0.277 & 0.153  \\
(A)       & \checkmark & -          & \checkmark & \checkmark & 0.417  & 0.265  & 0.180  & 0.127  & 0.305 & 0.167  \\
(B)       & \checkmark & \checkmark & -          & \checkmark & 0.420  & 0.266  & 0.180  & 0.127  & 0.304 & 0.168  \\
(C)       & \checkmark & \checkmark & \checkmark & -          & 0.418  & 0.266  & 0.181  & 0.129  & 0.308 & 0.169  \\ \hline
(D) & \checkmark & \checkmark & \checkmark & \checkmark & \textbf{0.437} & \textbf{0.279} & \textbf{0.191} & \textbf{0.137} & \textbf{0.310} & \textbf{0.175} \\ \hline
\end{tabular}%
}
\end{table}

==> rebuttal/table_cascade.tex <==
\begin{table}[]
\centering
\caption{The effect of a cascade of $N$ correction modules}
\label{rebuttal:cascade}
\resizebox{0.80\columnwidth}{!}{%
\begin{tabular}{c|cccccc}
\hline
$N$ & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & RG-L  & METEOR \\ \hline
1 & \textbf{0.437} & \textbf{0.279} & \textbf{0.191} & \textbf{0.137} & \textbf{0.310} & \textbf{0.175} \\
2         & 0.426  & 0.268  & 0.180  & 0.127  & 0.304 & 0.168  \\
3         & 0.413  & 0.264  & 0.182  & 0.131  & 0.300 & 0.167  \\
4         & 0.412  & 0.261  & 0.178  & 0.128  & 0.304 & 0.164  \\ \hline
\end{tabular}%
}
\end{table}

==> rebuttal/table_new_metric.tex <==
\begin{table}[]
\centering
\caption{An evaluation on new metrics on MIMIC-CXR.}
\label{rebuttal:new_metrics}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{c|cc}
\hline
Model           & BERT Score & RadGraph F1 \\ \hline
DART (Ours)     & 0.877      & 0.400       \\ \hline
\end{tabular}%
}
\end{table}

==> rebuttal/table_nlg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{An additional comparison in descriptive accuracy with the LLM-based methods [49,51]  on MIMIC-CXR and IU X-ray.}
\label{rebuttal:nlg}
\resizebox{\columnwidth}{!}{%
{
\begin{tabular}{c|c|c|cccccc}
\hline
Dataset                   & Method          & \# Params & BLEU-1         & BLEU-2         & BLEU-3         & BLEU-4         & ROUGE-L        & METEOR         \\ \hline
\multirow{3}{*}{MIMIC-CXR}                     & Yan et al. [51] & 175B     & -              & 0.180          & -              & -              & -              & -              \\
                                               & I3 + C2FD [49]  & 14.2B    & 0.402          & 0.262          & 0.180          & 0.128          & 0.291          & \textbf{0.175} \\ \cline{2-9} 
                                               & DART (Ours)     & 0.15B    & \textbf{0.437} & \textbf{0.279} & \textbf{0.191} & \textbf{0.137} & \textbf{0.310} & \textbf{0.175} \\ \hline
\multirow{2}{*}{IU X-ray} & I3 + C2FD [49]  & 14.2B    & \textbf{0.499} & 0.323          & 0.238          & 0.184          & 0.390          & \textbf{0.208} \\ \cline{2-9} 
                          & DART (Ours)     & 0.15B    & 0.486          & \textbf{0.348} & \textbf{0.265} & \textbf{0.208} & \textbf{0.411} & 0.205          \\ \hline
\end{tabular}%
}
}
\end{table}

==> sec/fig_ablation.tex <==
\begin{figure}[]
	\begin{center}
		\includegraphics[width=\linewidth]{res/fig_ablation.png}
	\end{center}
	\caption{We evaluate the effect of (a) the coefficient of correction loss ($\lambda_c$) and (b) the number of top-K retrieved text features ($K$) in our proposed method on BLEU-4 performance.}
	\label{fig:ablation}
\end{figure}
